ARGUS: Role-Aware Event Knowledge Graphs for U.S. Employment-Discrimination Complaints

U.S. employment-discrimination complaints describe complex event sequences that are not explicitly captured by lexical or embedding-based representations alone. We present ARGUS, a source-grounded pipeline that combines a 5W1H-inspired schema, legal-domain models, and LLM-based structured generation to construct document-level Event Knowledge Graphs (EKGs) from CourtListener complaints. ARGUS extracts fact-bearing statements, builds chunk-level event graphs with participant, temporal, and causal structure, and merges them into document-level representations. We evaluate graph quality through human and multi-model assessment and test downstream utility on claim classification and legal QA. The graph-structured classifier outperforms raw and linearized baselines on the held-out set, and EKG-only retrieval improves document-scoped QA, while open-retrieval gains remain limited by low first-stage candidate recall. These results suggest that EKGs are most useful for organizing and reasoning over evidence once relevant material has been retrieved.

==> recover.tex <==
\section{Experimental Setup}
\subsection{Datasets}
We collect employment-discrimination complaints (Nature of Suit 442, Civil Employment Cases) from CourtListener,\footnote{\url{https://www.courtlistener.com/}} an open legal-search repository maintained by the Free Law Project. The raw filings are OCR-derived scanned court documents with no existing gold labels for facts, events, or case similarity, so the corpus first passes through a Selenium-based scraping and cleaning pipeline:%(Appendix Figure~\ref{fig:data-pipeline}): 
document retrieval, OCR-to-text conversion, header/footer and boilerplate removal, section detection (isolating the FACTS narrative from jurisdictional and prayer-for-relief text), sentence segmentation, and normalization. To test robustness to jurisdiction-specific writing style, we draw 153 complaints from five U.S.\ district courts (Table~\ref{tab:dataset-stats}): Eastern District of Pennsylvania (EAPD), Eastern District of Kentucky (KYED), Southern District of New York (NYSD), Western District of Pennsylvania (PAWD), and District of Rhode Island (RID). Documents vary substantially in length and structure across districts.% (NYSD complaints average 6.91 chunks/document at 2{,}844 characters/chunk, roughly double EAPD's 4.35 chunks at 1{,}782 characters/chunk), and, where sentence-level fact annotation has been completed, 
The fraction of sentences that qualify as facts (rather than procedural or boilerplate text) ranges from 81.7\% (KYED) to 93.0\% (PAWD), giving a sense of how much of each filing is actually narrative signal. All splits are fixed at the document level to avoid boilerplate/near-duplicate leakage; fact extraction is supervised at the sentence level but inherits its parent document's split, while mini-graph extraction and merging are inference-only.

\begin{table}[h]
\centering
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\textbf{District} & \textbf{Docs} & \textbf{Chunks} & \textbf{Avg/Doc} & \textbf{Sentences} & \textbf{Fact Rate} \\
\midrule
EAPD & 20 & 87  & 4.35 & --    & --     \\
KYED & 31 & 138 & 4.45 & 1{,}155 & 81.7\% \\
NYSD & 46 & 318 & 6.91 & 4{,}808 & 92.7\% \\
PAWD & 28 & 165 & 5.89 & 1{,}607 & 93.0\% \\
RID  & 28 & 118 & 4.21 & 1{,}631 & 90.9\% \\
\bottomrule
\end{tabular}}
\caption{Dataset statistics across districts. Fact Rate = fraction of sentences labeled Fact (sentence-level annotation not yet completed for EAPD).}
\label{tab:dataset-stats}
\end{table}

\subsection{Evaluation of Graphical Components}
% \paragraph{Fact extraction.} We optimized our fact extraction component using document-level splits and a fixed held-out partition.%60/40 holdout. 
% Our primary metric is Micro-F1 with precision/recall and false-positive rate as supporting metrics \citep{kohavi-1995-crossval,powers-2011-evaluation}. LegalBERT trained on US data transfers to UK/India gold sets with F1 of 0.73/0.67 (Table~\ref{tab:cross_country}), outperforming LexLM. Compared to an LLM (GPT-5), LegalBERT gives higher precision while the LLM gives higher recall (Table~\ref{tab:bert_vs_llm}), a complementary pattern motivating our hybrid. On the US holdout, classifier-only and hybrid modes perform similarly (F1 0.87 LegalBERT / 0.86 LexLM), while the LLM-only mode is noticeably weaker (F1 $\approx$0.71--0.72, Table~\ref{tab:us_holdout}).

% \begin{table}[h]
% \centering
% \small
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Metric} & \textbf{UK-LB} & \textbf{IND-LB} & \textbf{UK-LX} & \textbf{IND-LX} \\
% \midrule
% Precision & 0.8889 & 0.7391 & 0.8000 & 0.6923 \\
% Recall    & 0.6154 & 0.6071 & 0.6154 & 0.6429 \\
% F1        & 0.7273 & 0.6667 & 0.6957 & 0.6667 \\
% \bottomrule
% \end{tabular}}
% \caption{Cross-country evaluation (trained on US data). LB=LegalBERT, LX=LexLM.}
% \label{tab:cross_country}
% \end{table}

% \begin{table}[h]
% \centering
% \small
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llcccc}
% \toprule
% \textbf{Data} & \textbf{Model} & \textbf{Acc.} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1} \\
% \midrule
% UK  & LegalBERT   & 0.9400 & 0.8889 & 0.6154 & 0.7273 \\
% UK  & LLM (GPT-5) & 0.8500 & 0.4615 & 0.9231 & 0.6154 \\
% IND & LegalBERT   & 0.8300 & 0.7391 & 0.6071 & 0.6667 \\
% IND & LLM (GPT-5) & 0.8800 & 0.7500 & 0.8571 & 0.8000 \\
% \bottomrule
% \end{tabular}}
% \caption{LegalBERT vs.\ LLM (GPT-5) on UK/IND data.}
% \label{tab:bert_vs_llm}
% \end{table}

% \begin{table}[h]
% \centering
% \small
% \begin{tabular}{lcc}
% \toprule
% \textbf{Mode} & \textbf{LegalBERT} & \textbf{LexLM} \\
% \midrule
% Classifier & 0.8718 & 0.8616 \\
% Hybrid     & 0.8711 & 0.8627 \\
% LLM        & 0.7115 & 0.7186 \\
% \bottomrule
% \end{tabular}
% \caption{US holdout (20\%) evaluation by pipeline.}
% \label{tab:us_holdout}
% \end{table}

\paragraph{Fact extraction.} We select LegalBERT and LexLM as legal-domain pretrained encoders from complementary BERT and RoBERTa model families, and fine-tune both for sentence-level Fact/Non-Fact classification. We compare them with a prompted GPT-5 baseline on the same fixed 100-sentence samples from the UK and Indian gold datasets (Table~\ref{tab:fact-cross-jurisdiction}). Our primary metric is Micro-F1, with accuracy, precision, and recall reported as supporting metrics \citep{kohavi-1995-crossval,powers-2011-evaluation}. LegalBERT reaches the highest encoder F1 on the UK sample (0.7273), whereas GPT-5 achieves higher recall on both samples and the highest F1 on the Indian sample (0.8000). This complementary precision--recall behavior motivates our hybrid fallback. On the U.S.\ holdout, classifier-only and hybrid modes perform similarly (F1 0.87 LegalBERT / 0.86 LexLM), while the LLM-only mode is noticeably weaker (F1 $\approx$0.71--0.72, Table~\ref{tab:us_holdout}).

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
\textbf{Data} & \textbf{Model} & \textbf{Acc.} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1} \\
\midrule
UK    & LegalBERT & 0.9400 & 0.8889 & 0.6154 & 0.7273 \\
UK    & LexLM     & 0.9300 & 0.8000 & 0.6154 & 0.6957 \\
UK    & GPT-5     & 0.8500 & 0.4615 & 0.9231 & 0.6154 \\
\midrule
India & LegalBERT & 0.8300 & 0.7391 & 0.6071 & 0.6667 \\
India & LexLM     & 0.8200 & 0.6923 & 0.6429 & 0.6667 \\
India & GPT-5     & 0.8800 & 0.7500 & 0.8571 & 0.8000 \\
\bottomrule
\end{tabular}}
\caption{Fact-extraction results on fixed 100-sentence UK and Indian samples. LegalBERT and LexLM are fine-tuned legal-domain encoders; GPT-5 is a prompted baseline. All metrics treat Fact as the positive class.}
\label{tab:fact-cross-jurisdiction}
\end{table}

\paragraph{Mini-graph extraction.} On a fixed 24-chunk evaluation set, Claude Sonnet 4.5 + GEPA achieves near-perfect structural reliability (schema validity, coverage all 1.0) and a quality score of 0.896, with causal self-loops as the main residual error. Comparing open-source alternatives (Table~\ref{tab:open_source_minigraph}), Qwen achieves higher semantic quality and richer, cheaper graphs than GPT-OSS-120B, which is slightly stronger structurally. For \textbf{human evaluation}, all four team members independently reviewed each chunk-level mini-graph alongside its source text through a lightweight annotation dashboard (Appendix Figure~\ref{fig:annotation_dashboard}), assigning one of three labels (\emph{Aligned}, \emph{Partially Aligned}, or \emph{Misaligned}) plus a free-text reasoning note and, when not fully aligned, an error tag (e.g., missing event, wrong role, hallucinated detail). We aggregate labels with Percent Agreement, Fleiss' $\kappa$, and Krippendorff's $\alpha$ (nominal and ordinal) across annotators (Table~\ref{tab:human_minigraph_alignment}). The evaluated FrameNet-guided Qwen configuration reaches 85.2\% Aligned with substantial inter-annotator agreement (Fleiss' $\kappa=0.669$), versus 78.3\% Aligned and ($\kappa=0.143$) for the evaluated Claude configuration. Because the models and the use of frame guidance change together, this is a configuration-level comparison and isolate the causal effect of FrameNet guidance. %without frame guidance, suggesting that constraining extraction to a fixed frame vocabulary improves not just raw alignment but also how consistently different human raters judge that alignment.

\begin{table}[h]
\centering
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|lcc}
\toprule
\textbf{Metric} & \textbf{GPT} & \textbf{Qwen} & \textbf{Metric} & \textbf{GPT} & \textbf{Qwen} \\
\midrule
Quality Score & 0.8272 & 0.8852 & Events/Chunk & 7.09 & 7.50 \\
Judge Score & 0.6642 & 0.7966 & Temporal Edges/Chunk & 2.15 & 3.12 \\
Structural Score & 0.9902 & 0.9739 & Causal Edges/Chunk & 1.00 & 2.29 \\
Temporal Consist. & 0.9118 & 0.7647 & Schema Validity & 1.00 & 1.00 \\
\bottomrule
\end{tabular}}
\caption{Open-source model comparison for mini-graph extraction.}
\label{tab:open_source_minigraph}
\end{table}

\begin{table}[h]
\centering
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|lcc}
\toprule
\textbf{Metric} & \textbf{Claude} & \textbf{Qwen} & \textbf{Metric} & \textbf{Claude} & \textbf{Qwen} \\
\midrule
Aligned & 78.30\% & 85.20\% & Percent Agree. & 69.60\% & 91.70\% \\
Partially Aligned & 17.40\% & 14.80\% & Fleiss' $\kappa$ & 0.143 & 0.669 \\
Misaligned & 4.30\% & 0.00\% & Krippendorff $\alpha$ & 0.153 & 0.673 \\
\bottomrule
\end{tabular}}
\caption{Human annotation of mini-graph alignment.}
\label{tab:human_minigraph_alignment}
\end{table}

\paragraph{Event-graph merging.} As a baseline, we prompt Claude Sonnet 4.5 (via the Keymaker API) to generate a document-level EKG directly from the full FACTS section in a single pass, with no chunking, intermediate structure, or multi-stage merge: one prompt, one graph per document. The exact one-shot prompt is shown in Appendix B.1.
%\begin{quote}
%\small\ttfamily
%"You are a legal event extraction analyst. You are given one full legal document with sentence-labeled facts. Extract ONE overall document-level event graph, just extract what you think are events. Return strict JSON only. Schema requires: entities, events, temporal\_edges, causal\_edges with consistent IDs (E1..En, EV1..EVn). Events are the only nodes; entities attach to events as participants. Temporal relations: BEFORE, SAME\_TIME. Causal relation: CAUSES, ENABLES."
%\end{quote}
This one-shot baseline fails completely on 2 of 5 documents (zero events extracted) and varies widely in coverage and structure on the rest (Table~\ref{tab:baseline_onshot}), reflecting the difficulty of jointly performing event detection, role assignment, and relational reasoning over a long legal document in a single pass, and motivating our staged pipeline, which decomposes extraction and enforces structure through chunk-level mini-graphs and controlled merging. Using three LLM judges (DeepSeek-R1, Qwen3-Coder, Mistral-Large), our hybrid graphs are preferred over the baseline with perfect win rate/agreement/AC1 \citep{gwet2008computing} on evidence grounding, edge correctness, and overall quality, and a 93.3\% win rate on event grounding (all $p=0.031$, Table~\ref{tab:inter_model}); intra-model stability under temperature variation is 100\% for Qwen/Mistral and 80\% for DeepSeek-R1 (Table~\ref{tab:intra_model}).

\begin{table}[h]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Case} & \textbf{Events} & \textbf{Temporal} & \textbf{Causal} \\
\midrule
Miczulski v. Alix Inc & 21 & 19 & 6 \\
Poole v. Ampler Pizza & 0 & 0 & 0 \\
Sermarini v. A Step Up & 16 & 14 & 20 \\
Bleiler v.\ Chester Co. & 0 & 0 & 0 \\
Bacon v.\ M.A.G. Ent. & 17 & 16 & 13 \\
\bottomrule
\end{tabular}
\caption{One-shot LLM baseline event-graph extraction.}
\label{tab:baseline_onshot}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Dimension} & \textbf{Win} & \textbf{Agree.} & \textbf{AC1} & \textbf{$p$} \\
\midrule
Event Grounding  & 93.3\% & 86.7\% & 0.848 & 0.031 \\
Proper Evidence  & 100\%  & 100\%  & 1.0   & 0.031 \\
Edge Correctness & 100\%  & 100\%  & 1.0   & 0.031 \\
Overall          & 100\%  & 100\%  & 1.0   & 0.031 \\
\bottomrule
\end{tabular}
\caption{Inter-model evaluation across LLM judges.}
\label{tab:inter_model}
\end{table}

%\begin{table}[h]
%\centering
%\small
%\begin{tabular}{lccc}
%\toprule
%\textbf{Model} & \textbf{Stability} & \textbf{Flip} & %\textbf{AC1} \\
%\midrule
%DeepSeek & 80\%  & 20\% & 1.0 \\
%Qwen     & 100\% & 0\%  & 1.0 \\
%Mistral  & 100\% & 0\%  & 1.0 \\
%\bottomrule
%\end{tabular}
%\caption{Intra-model stability under temperature %variation.}
%\label{tab:intra_model}
%\end{table}

The full table showing temperature stability is found in Appendix B.2.
